Detecting Buggy Contracts via Smart Testing

Smart contracts are susceptible to critical vulnerabilities. Hybrid dynamic analyses, such as concolic execution assisted fuzzing and foundation model assisted fuzzing, have emerged as highly effective testing techniques for smart contract bug detection recently. This hybrid approach has shown initial promise in real-world benchmarks, but it still suffers from low scalability to find deep bugs buried in complex code patterns. We observe that performance bottlenecks of existing dynamic analyses and model hallucination are two main factors limiting the scalability of this hybrid approach in finding deep bugs. To overcome the challenges, we design an interactive, self-deciding foundation model based system, called SmartSys, to support hybrid smart contract dynamic analyses. The key idea is to teach foundation models about performance bottlenecks of different dynamic analysis techniques, making it possible to forecast the right technique and generates effective fuzz targets that can reach deep, hidden bugs. To prune hallucinated, incorrect fuzz targets, SmartSys feeds foundation models with feedback from dynamic analysis during compilation and at runtime. The interesting results of SmartSys include: i) discovering a smart contract protocol vulnerability that has escaped eleven tools and survived multiple audits for over a year; ii) improving coverage by up to 14.3\% on real-world benchmarks compared to the baselines.

==> Tables/FP.tex <==
\begin{table}[!t]
\caption{Analysis on reported bugs. TP: true positive; FP: false positive; FN: false negative; ER: error; TO: timeout; TP Ratio: true positive ratio of reported bug;  Analysis Ratio: the number of contracts successfully analyzed by a given tool without errors or timeouts.}
\label{table:reported_bugs}
\rowcolors{2}{white}{gray!30}
\footnotesize
\setlength{\tabcolsep}{2.5pt}
\centering
\renewcommand{\arraystretch}{1.2}
\scalebox{0.73}{
\begin{tabular}{l|l|l|l|l}
\hline
                        & \sys   & \ilfnq & \smartestnq & \teethernq \\ \hline
TP                      & 3,054  & 117    & 664         & 432        \\
FP                      & 0      & 0      & 911         & 12         \\
FN                      & 122    & 109    & 648         & 0          \\
ER                      & 33     & 1,785  & 3,391       & 1,007      \\
TO                      & 10     & 21     & 8           & 2,031      \\ \hline
\textbf{TP Ratio}       & 100\%   & 100\%   & 37.10\%      & 97.21\%     \\
\textbf{Analysis Ratio} & 99.78\% & 90.80\% & 82.68\%      & 84.52\%     \\ \hline
\end{tabular}}\end{table}


==> Tables/bug.tex <==
\begin{table}
\subfloat[Reported bugs breakdown by type from sampled 19,621 SmartBugs benchmark contracts.]{
\label{table:reported_bugs}

\footnotesize
\setlength{\tabcolsep}{2.5pt}
%\centering
\renewcommand{\arraystretch}{1.2}
%\scalebox{0.73}{
\begin{tabular}{l|l|l|l|l}
\hline
Bug Type               & \sys  & \ilfnq & \smartestnq & \teethernq \\ \hline
Reentrancy             & 301   & 0    & 0           & 0          \\
Integer Over/underflow & 749   & 0    & 911         & 0          \\
Arithmetic Flaw        & 633   & 0    & 648         & 0          \\
Suicidal Contract      & 209   & 33   & 132         & 273        \\
Ether Leakage          & 611   & 21   & 82          & 93         \\
Ether Lock             & 57    & 63   & 0           & 0          \\
Access Control         & 494   & 0    & 12          & 78         \\ \hline
\textbf{Total Bugs}    & 3,054 & 117  & 1,785       & 444        \\ \hline
\end{tabular}}
\quad
\subfloat[Analysis on reported bugs. TP: true positive; FP: false positive; FN: false negative; ER: error; TO: timeout; TP Ratio: true positive ratio of reported bug;  Analysis Ratio: the number of contracts successfully analyzed by a given tool without errors or timeouts.]{
\label{table:bug_analysis}

\footnotesize
\setlength{\tabcolsep}{2.5pt}
%\centering
\renewcommand{\arraystretch}{1.2}
%\scalebox{0.73}{
\begin{tabular}{l|l|l|l|l}
\hline
                        & \sys   & \ilfnq & \smartestnq & \teethernq \\ \hline
TP                      & 3,054  & 117    & 664         & 432        \\
FP                      & 0      & 0      & 910         & 12         \\
FN                      & 0    & 109    & 648         & 53          \\
ER                      & 33     & 1,785  & 74     & 569      \\
TO                      & 10     & 1086     & 801          & 2,031      \\ \hline
\textbf{TP Ratio}       & 100\%   & 100\%   & 37.10\%      & 97.21\%     \\
\textbf{Analysis Ratio} & 99.78\% & 35.06\% & 71.77\%      & 83.95\%     \\ \hline
\end{tabular}}
\end{table}

==> Tables/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

The recent state-of-the-art in smart contracts has advanced towards a wide array of dynamic analyses, with impressive results achieved by fuzzing \cite{fuzzingsurvey} and concolic execution \cite{concolicexe, learnedfuzzing} particularly. Fuzzing and concolic execution often require substantial computational resources (CPU, memory, and runtime). However, no single technique is perfect for detecting diverse types of smart contract bugs. This begets the scalability question: what if we can automatically forecast the right technique to use before heavily investing scarce computational resources?  

In addition to resource constraints, new studies show that bugs are often buried deep within execution paths \cite{arbiter}, and more importantly, detecting such ``deep bugs'' requires reasoning across multi-modal information, \ie source (or binary) code and natural language hints \cite{smartinv}. Unfortunately, existing tools \cite{sailfish, securify, ethbmc} can reason about a single modality (source or binary code) only. The lack of multi-modal reasoning misses a panoply of ``deep bugs'' hidden in execution paths and multi-modal information. This begets the coverage question: how can we reason across multi-modal sources of information to reach ``deep bugs'' of diverse types?

Our research seeks to answer the scalability and coverage questions in real world smart contract applications.
While current improvement presents valuable ways forward, dynamic analyses come at the cost of multi-modal reasoning and have inherent limitations. Scalable analyses, \eg randomized fuzzing, suffer from low code coverage, because fuzzers that generate random inputs frequently get stuck on constrained paths. High code coverage analyses, \eg concolic execution and coverage optimized fuzzing, often comes at the price of limited scalability, because their exhaustive path searches either focus on a small subset of code or require exponentially growing memory space \cite{pathexplosion}.

Existing static analyses \cite{slither, smartcheck} have also attempted to address the scalability issue by offering precise graph representations of program control flows. Despite higher precision, static analyses similarly lack multi-modal reasoning capability and the ability to exhaustively search paths that can discover potential vulnerabilities. Thus, static analyses suffer from low coverage in terms of both program code and detectable bug types. 

We demonstrate that it is feasible to achieve both high scalability and high coverage analysis by first forecasting the suitable techniques and then learning to reason about multi-modal information, \eg source code, natural language hints, and documentations. A program analysis technique is most useful when it can reason about domain-specific knowledge and detect diverse types of bugs in an automated fashion. Towards that goal, we propose a fully automated, multi-modal learning framework that can forecast the right technique based on un-covered code and generate test targets via learning from multimodal information. 

To achieve high scalability, our key insight is that foundation models fine-tuned on domain specific data can reasonably forecast the right technique within seconds, thereby saving multiple CPU days that might have gone to futile techniques. To achieve high coverage, our key insight is that prompting pre-trained foundation models in contexts can generate test targets localizing ``deep bugs'' hidden in execution paths and multi-modal information. 

To evaluate our proposed framework, we have built \sys and evaluated it on real world smart contract benchmarks used in blockchain industry, demonstrating that \sys improved coverage by up to 14.3\% on those benchmarks. Interestingly, \sys has discovered a critical vulnerability that has escaped eleven existing tools for more than a year. We immediately reported the vulnerability to the developers (at the time of submission) and are anticipating their confirmation. \junfeng{has the bug been confirmed? if not, please try to follow up and get the bug confirmed.}

\vspace{.1cm}\noindent\textbf{Contributions.} We make the following contributions:
\begin{itemize}[leftmargin=*]
\item To the best knowledge of our knowledge, \sys is the first interactive model system that can reason about multi-modal inputs to achieve \textit{both} high scacalability and high coverage in testing real world smart con
\item \sys unites foundation models' multi-modal learning capability with the soundness of concolic execution guided fuzzing, generating test cases (seeds) that consistently improve \efcf's coverage, an AFL++ adapted fuzzer for Solidity, on sampled 115 projects.

\item we present a new benchmark, comprised of contracts that reflect the top ten types of commonly exploited zero-day vulnerabilities from 2022-2024. 

\item Our evaluation shows that \sys is highly versatile, adaptable to other fuzzing and concolic execution modules. 

\end{itemize}


==> Tables/motivation_techniques.tex <==
\begin{table}[!t]
\footnotesize
\centering
\renewcommand{\arraystretch}{1.1}
 \caption{\textbf{Capability comparisons between \sys and related tools. We note whether a tool has high scalability through the combined use of static and dynamic techniques, has high coverage on contract source code, supports inter-function analysis, supports inter-contract analysis, has symbolic reasoning capabilities, has multimodal reasoning capabilities, detects diverse types of bugs on real-world contracts. \halfcirc: partial capability in limited settings.}}
\begin{tabular}{lccccccc}
  Tools  & \rot{High Scalability}
    & \rot{High Coverage}
    & \rot{Inter-Function}
     & \rot{Inter-Contract}
    & \rot{Symbolic Reasoning}
    & \rot{Multi-modal Reasoning}
    & \rot{Diverse Bugs}\\
    \midrule
\slither & \n  & \n & \halfcirc  & \n & \n & \n & \n\\
\ilf & \halfcirc  & \halfcirc & \y  & \n & \n & \n & \halfcirc\\
\efcf &  \halfcirc & \n & \n  & \y & \n & \n  & \n\\
\echidna &  \halfcirc & \n & \n & \n & \n & \n & \n\\
\teether & \n & \n & \halfcirc   & \n & \y & \n  & \n\\
\ethbmc & \n & \n  & \halfcirc & \halfcirc & \y & \n  & \n\\
\sailfish & \y & \n & \halfcirc  & \y & \y & \n  & \n\\
\smartest & \n & \n & \n  & \n & \y & \n & \n\\
\verismart & \n & \n & \n  & \n & \n & \n & \n\\
\verisol & \n & \n & \halfcirc & \y & \n & \n & \y\\
\verx & \n & \n & \n  & \y & \y & \n & \n\\
\sys & \y & \y  & \y & \y & \y & \y  & \y\\
    \bottomrule
\end{tabular}
\label{tab:motivating_techniques}
\end{table}

==> Tables/overview.tex <==
\section{Overview}
\label{sec:overview}

\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{Fig/arch.drawio.pdf}
\caption{\sys's workflow: }
\label{Fig:overview}
\end{figure}

Fig.~\ref{Fig:overview} illustrates our efforts to build such an intelligent system and the workflow of \sys. During fine-tuning, the fuzz scanner generates coverage reports from training contracts (\textcircled{\footnotesize{1}}). \sys automatically processes these reports to fine-tune the forecast model. Once the forecast model is fully fine-tuned (\textcircled{\footnotesize{2}}), \sys calls the forecast model after the fuzz scanner generates a coverage report on a previously unseen input contract (\textcircled{\footnotesize{3}}). Then the forecast model decides whether to invoke concolic execution or the generator model (\textcircled{\footnotesize{4}}). If the generator model is invoked, \sys feeds model generated test targets back into the fuzz scanner (\textcircled{\footnotesize{5}}). \sys repeats this process until coverage plateaus or the fuzz scanner time outs. Then \sys outputs possible exploits (test cases) from the fuzz scanner (\textcircled{\footnotesize{6}}). If concolic execution is invoked, \sys uses concolic execution's output as possible exploits (test cases) (\textcircled{\footnotesize{6}}). 

Each module is optimized towards generating test cases that can discover bugs embedded in deep code state. 
Specifically, \sys's three novel modules, which fundamentally differ from existing tools \cite{smartest, verx, manticore, smartian, solsee, learnedfuzzing, sailfish, contractfuzzer}, are the following: 

\vspace{0.1cm}\textbf{Forecast Model.} The fine-tuned model takes coverage report and smart contract source code as input and predicts the next module \ie concolic execution or test case generation model, as output. If the binary prediction model predicts 0 (meaning that the model predicts concolic execution as a befitting module to overcome the coverage plateaus), \sys proceeds to the concolic execution module as a next step. If the binary prediction model predicts 1 (meaning that the model predicts foundation model as a befitting module to overcome the coverage plateaus), \sys proceeds to prompt the generator model as the next step to generate test targets (details in \S\ref{subsec: fine-tuned Binary Classification Model}).
%\sys employs different default foundation models for binary classification and test case generation for optimal performance. The technical rationale and performance-based evidence for such design choice are detailed in \ref{subsec: Finetuned Binary Classification Model}. 

\vspace{0.1cm}\textbf{Optimized Concolic Execution.} To escape coverage plateaus, \sys employs coverage-guided concolic execution to generate test cases with real-time coverage monitoring. This module takes a smart contract, initial corpus, and coverage report as input and returns new test cases and updated coverage as output. Although concolic (or symbolic) execution has been widely used for test case generation in other domains such as C and Java \cite{Klee, ucklee, dart, multise}, Ethereum smart contracts and solidity require technical optimizations to maximize coverage and to detect hidden bugs. We will detail each of these techniques in \S\ref{subsec: Optimized Concolic Execution}. 

\vspace{0.1cm}\textbf{Generator Model.} The test harness generator model takes smart contract source code and coverage report as input and generates test harnesses as output. When \sys prompts the model, the goals are: i) to generate test harnesses that can maximize coverage for the uncovered functions; ii) to generate test harnesses with specific function invocation orders that can discover hidden bugs. To achieve the two goals, we designed two distinct sets of prompts uniquely tailored to the tasks. the first set of prompts is a four-step iterative prompting process that provides precise contexts and parameter setup for test harness generation. The second set of prompts aims to find specific function invocation orders that can detect hidden bugs. 
After extracting specific function invocation orders and functions not covered by initial fuzzing, We will detail the prompts and test harness generation, and test cases conversion process in \S\ref{subsec: Test Case Generation Model}.
%\kexin{step 6: justify LLM or symbolic execution makes sense; separate function invocation order and input value generation; if we use a fixed function and not efficient; else: if we need function invocation orders and efficienty; reverse explaining: after training, we discover that LLMs are good at identifying invocation order and more efficient covering constraints test case. When we have multiple function invocation order, predicting 1.}

==> Tables/related_work.tex <==
\begin{table*}[!t]
\small
\setlength{\tabcolsep}{6pt}
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lllllllll}
\toprule
\textbf{Technique} & \textbf{Genre} & \textbf{Coverage} & \textbf{Scalability} & \textbf{Manual Effort} & \textbf{Bug Types} & \textbf{FP} & \textbf{FN} & \textbf{Examples} \\
\midrule
Graph-based & static & low & low & rules, queries & limited & medium & high & \cite{slither,staticsymbolic, smartcheck, ethor} \\

Static taint & static & low & low & rules, inputs  & limited & high & low & \cite{osiris, mythril} \\

Dynamic taint & dynamic & low & low & rules, inputs  & limited & low & high & \cite{etainter, etherolic, actualtaint, dynamictaint} \\

Fuzzing & dynamic & low & medium & harness, oracles & limited & low & high & \cite{echidna, sfuzz, efcf, contractfuzzer} \\

Conc. exe. & dynamic & medium & low & rules, env. modeling  & limited & low & high & \cite{teether, ethbmc, ethploit, smartest} \\

CE-assis. fuzzing & dynamic & high & low & rules, env. modeling & limited & low & high & \cite{learnedfuzzing, oyente, confuzzius, beak} \\

\sys & hybrid & high & high & None & generic & low & low & N/A \\

\bottomrule
\end{tabular}
\caption{Taxonomy on the pros and cons of common smart contract testing techniques. ``Conc. exe.'' refers to concolic execution. ``CE-assis. fuzzing'' refers to concolic execution assisted fuzzing. ``Manual Effort'' refers to required manual instrumentations, \eg ``rules'' refers to human constructed graph querying rules; ``queries'' refers to queries over a graph representation; ``inputs'' refer to human constructed test inputs; ``oracle'' as instrumented test oracles for fuzzing; ``env. modeling'' as environment modeling for concolic execution.  ``FP'' and ``FN'' refers to false positives and false negatives respectively. %\kexin{why LLM? library function calls - unknown func{...} cannot track this. external func calls are manual efforts. why quantization forgets about certain knowledge??}}
\label{tab:related_work}
\end{table*}

==> Tables/remove.tex <==
\begin{table}[!t]
\footnotesize
\setlength{\tabcolsep}{8pt}
\centering
\renewcommand{\arraystretch}{1.1}
\caption{\textbf{Multi-modality analysis for the forecast model.}}
\label{table:remove}


\begin{tabular}{lllll}
\toprule
Features & Acc. & Prec. & Rec.  & F1 \\
 \midrule
% \midrule
\rowcolor{gray!30}
w/o NL & 0.82  & 0.81 & 0.73 & 0.71\\
% \bottomrule
% \midrule
 \cite{falcon} & 0.81  & 0.81 & 0.70  & 0.75\\
% \bottomrule
\bottomrule
\end{tabular}
\end{table}

==> Tables/symbolic_training.tex <==
\begin{table*}[!t]
\footnotesize
\setlength{\tabcolsep}{1.2pt}
\centering
\renewcommand{\arraystretch}{1.1}
\caption{Extracted features from symbolic execution traces for finetuing pre-trained model and guiding future symbolic execution during inference.}
\label{table:ground truth}
\begin{tabular}{lll}
\toprule[.6pt]
\textbf{Features} & \textbf{Modalities} &\textbf{Rationale} \\ 
\midrule[.6pt]
Path Constraints  & Bytecode
    & Repeating same path constraints under different executions suggests\\
 & 
    & potentially redundant states\\
 \midrule[.6pt]   
Executed Paths  & Natural Language(Numbers)
   & useful for tracking new paths that have not been repeated and\\
 & 
    & are likely to increase coverage\\
 \midrule[.6pt]   
Targeting Instr.  & Natural Language(Numbers)
    & Targeting instructions not covered by previously executed paths\\ 
 & & can increase coverage\\
\midrule[.6pt]
Coverage  & Natural Language(Numbers)
    & real-time coverage update measures how effective an executed path and\\ &   
    & test cases are in improving coverage during each iteration\\
\midrule[.6pt]
Tx Sequences & Source Code
    & useful for monitoring coverage, computing scoring function, and\\ &
    & the length of transactions required to reach new code\\

\bottomrule[.6pt]
\end{tabular}
\end{table*}

==> background.tex <==
\section{Background and Related Work}
\label{sec:relwork}
In~\secref{sec:intro} you talked about the project at a very high-level. This is
the section from where you will start giving details. First with things that are
already done, and familiarize the reader with background information they will
need to understand you work. 


\paragraph{Threat model.}
Often this section you will discuss the threat-model, but there is no strict consensus on that. 


Here is how you cite papers. For example, we read papers in the
class~\cite{rahul2016pwtypos,dodisetal:2004}.  And here is some random citation~\cite{Bojinov:2010:KLP,schechter:2010:pen,everspaugh2015pythia,bellare2009format,Juels:2014}


\subsection{Overview of the design}
\label{sec:overview}

And then just to showoff some \LaTeX skills, here is a Tikz plot.
\input{images/mainflow.tex}

You refer to a figure in the following way. In~\figref{fig:mainflow} we show
some thing that is relevant for the Multisketch paper by Chatterjee et
al.~\cite{chatterjee2019multisketches}. Add your bibliography to the
\textsf{bib.bib} file. You can copy the Bibtex format citation from Google
Scholar.


==> defs.tex <==
\usepackage{xparse}
\newcommand{\bnm}{\begin{newmath}}
\newcommand{\enm}{\end{newmath}}

\newcommand{\bea}{\begin{eqnarray*}}%
\newcommand{\eea}{\end{eqnarray*}}%

\newcommand{\bne}{\begin{newequation}}
\newcommand{\ene}{\end{newequation}}

\newcommand{\bal}{\begin{newalign}}
\newcommand{\eal}{\end{newalign}}

\newenvironment{newalign}{\begin{align}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{align}}

\newenvironment{newmath}{\begin{displaymath}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{displaymath}}

\newenvironment{neweqnarrays}{\begin{eqnarray*}%
\setlength{\abovedisplayskip}{-4pt}%
\setlength{\belowdisplayskip}{-4pt}%
\setlength{\abovedisplayshortskip}{-4pt}%
\setlength{\belowdisplayshortskip}{-4pt}%
\setlength{\jot}{-0.4in} }{\end{eqnarray*}}

\newenvironment{newequation}{\begin{equation}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{equation}}


\newcounter{ctr}
\newcounter{savectr}
\newcounter{ectr}

\newenvironment{newitemize}{%
\begin{list}{\mbox{}\hspace{5pt}$\bullet$\hfill}{\labelwidth=15pt%
\labelsep=4pt \leftmargin=12pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{3pt} }}{\end{list}}


\newenvironment{newenum}{%
\begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr} \labelwidth=17pt%
\labelsep=5pt \leftmargin=22pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{2pt} }}{\end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Figure and table macros
%

\newcounter{mytable}
\def\mytable{\begin{centering}\refstepcounter{mytable}}
\def\endmytable{\end{centering}}

\def\mytablecaption#1{\vspace{2mm}
  \centerline{Table \arabic{mytable}.~{#1}}
  \vspace{6mm}
  \addcontentsline{lot}{table}{\protect\numberline{\arabic{mytable}}~{#1}}
}


\newcounter{myfig}
\def\myfig{\begin{centering}\refstepcounter{myfig}}
\def\endmyfig{\end{centering}}

\def\myfigcaption#1{
             \vspace{2mm}
             \centerline{\textsf{Figure \arabic{myfig}.~{#1}}}
             \vspace{6mm}
             \addcontentsline{lof}{figure}{\protect\numberline{\arabic{myfig}}~{#1}}}


\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}

\newcommand{\decOracle}{\textbf{Dec}}

\newcommand{\negsmidge}{{\hspace{-0.1ex}}}
\newcommand{\cdotsm}{\negsmidge\negsmidge\negsmidge\cdot\negsmidge\negsmidge\negsmidge}

\def\suchthatt{\: :\:}
\newcommand{\E}{{\rm I\kern-.3em E}}
\newcommand{\Prob}[1]{{\Pr\left[\,{#1}\,\right]}}
\newcommand{\Probb}[2]{{\Pr}_{#1}\left[\,{#2}\,\right]}
\newcommand{\CondProb}[2]{{\Pr}\left[\: #1\:\left|\right.\:#2\:\right]}
\newcommand{\CondProbb}[2]{\Pr[#1|#2]}
\newcommand{\ProbExp}[2]{{\Pr}\left[\: #1\:\suchthatt\:#2\:\right]}
\newcommand{\Ex}[1]{{\textnormal{E}\left[\,{#1}\,\right]}}
\newcommand{\Exx}{{\textnormal{E}}}
\newcommand{\given}{\ensuremath{\,\big|\,}}


\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\def\negl{\mathsf{negl}}


\newcommand{\secref}[1]{\mbox{Section~\ref{#1}}}
\newcommand{\appref}[1]{\mbox{Appendix~\ref{#1}}}
\newcommand{\thref}[1]{\mbox{Theorem~\ref{#1}}}
\newcommand{\defref}[1]{\mbox{Definition~\ref{#1}}}
\newcommand{\corref}[1]{\mbox{Corollary~\ref{#1}}}
\newcommand{\lemref}[1]{\mbox{Lemma~\ref{#1}}}
\newcommand{\clref}[1]{\mbox{Claim~\ref{#1}}}
\newcommand{\propref}[1]{\mbox{Proposition~\ref{#1}}}
\newcommand{\factref}[1]{\mbox{Fact~\ref{#1}}}
\newcommand{\remref}[1]{\mbox{Remark~\ref{#1}}}
\newcommand{\figref}[1]{\mbox{Figure~\ref{#1}}}
\renewcommand{\algref}[1]{\mbox{Algorithm~\ref{#1}}}
% \newcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
% Have to use \renewcommand because exists already in amsmath
\renewcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
\newcommand{\consref}[1]{\mbox{Construction~\ref{#1}}}
\newcommand{\tabref}[1]{\mbox{Table~\ref{#1}}}

\newcommand{\get}{{\:{\leftarrow}\:}}
\newcommand{\gett}[1]{\:{\leftarrow}_{#1}\:}
\newcommand{\getsr}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle\$$}}}\:}}
\newcommand{\getm}{{\:\leftarrow_{\mdist}\:}}
\newcommand{\getd}{{\:\leftarrow_{\ddist}\:}}
%\newcommand{\getm}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \mdist$}}}\:}}
\newcommand{\getk}{{\:\leftarrow_{\kdist}\:}}
%\newcommand{\getk}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \kdist$}}}\:}}
\newcommand{\getp}{{\:\leftarrow_{p}\:}}



\newcommand{\gamesfontsize}{\small}
\newcommand{\fpage}[2]{\framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}}
\newcommand{\mpage}[2]{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}

\newcommand{\hpages}[3]{\begin{tabular}{cc}\begin{minipage}[t]{#1\textwidth} #2 \end{minipage} & \begin{minipage}[t]{#1\textwidth} #3 \end{minipage}\end{tabular}}

\newcommand{\hpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #3 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #4 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #4 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #6 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagessss}[8]{
        \begin{tabular}{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #6 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #7 \end{minipage}
        &
        \begin{minipage}[t]{#4\textwidth}\gamesfontsize #8 \end{minipage}
        \end{tabular}
    }


\newcommand{\hfpages}[3]{\hfpagess{#1}{#1}{#2}{#3}}
\newcommand{\hfpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #3 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagessss}[8]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #7 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#4\textwidth}\setstretch{1.1}\gamesfontsize #8 \end{minipage}}
        \end{tabular}
    }

\newcommand{\vecw}{\mathbf{w}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\load}{L}
\newcommand{\coll}{\mathsf{Coll}}
\newcommand{\nocoll}{\overline{\mathsf{Coll}}}


\newcommand{\Img}{\textsf{Img}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Fonts and symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\funcfont{\textsf}
\newcommand\variablefont{\texttt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW COMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \Perm {\funcfont{Perm}}
\def \calC {{\mathcal{C}}}
\def \calU {{\mathcal{U}}}
\renewcommand{\u}{\ensuremath{u}}
\newcommand{\unew}{\ensuremath{\tilde{u}}}

\newcommand{\calN}{\mathcal{N}}
\def \sspace {{\mathcal{S}}}
\def \strings {{\mathcal{S}}}
\def \slen {{s}}
\def \kspace {{\mathcal{K}}}
\def \kspacesize {{m}}
\def \mspacesize {{n}}
\def \kdict {D}
\def \dictsize {d}
\newcommand{\kdist}{p_k}
\newcommand{\mdist}{\ensuremath{{W}}}
\newcommand{\alldist}{\rho}
\newcommand{\pwdist}{\transgen}
\newcommand{\ddist}{\rho_{dec}}
\newcommand{\PWset}{{\mathcal{P}}}  % TODO: fix, same as \pwdist
\newcommand{\PWsetvec}{\vec{\mathcal{P}}}
\newcommand{\PWvec}{\vec{P}}
\newcommand{\domvec}{\vec{D}}
\newcommand{\humanornot}{\vec{h}}
\newcommand{\dom}{\textsf{dom}}
%\def \kdist {{\kappa}}
%\def \mdist {{\mu}}
%\def \ddist {{\delta}}
\def \pspace {{\mathcal{P}}}
\def \mpspace {{\mathcal{MP}}}
\def \cspace {{\mathcal{C}}}
\def \key {\kappa}
\def \msg {M}
\def \seed {S}
\def \ctxt {C}
\def \ctxtpart {C_2}
\newcommand{\genprime}{{\textsf{GenPrime}}}
\newcommand{\isprime}{{\textsf{IsPrime}}}
\newcommand{\LeastLesserPrime}{{\textsf{PrevPrime}}}
\newcommand{\pwset}{\mathcal{S}}
\newcommand{\DTE}{{\textsf{DTE}}}
\newcommand{\encode}{{\textsf{encode}}}
\newcommand{\decode}{{\textsf{decode}}}

\newcommand{\DTEsingle}{{\textsf{1PW-DTE}}}
\newcommand{\encodesingle}{{\textsf{1PW-encode}}}
\newcommand{\decodesingle}{{\textsf{1PW-decode}}}

\newcommand{\DTErss}{{\textsf{RSS-DTE}}}
\newcommand{\encoderss}{{\textsf{RSS-encode}}}
\newcommand{\decoderss}{{\textsf{RSS-decode}}}

\newcommand{\DTEindep}{{\textsf{MPW-DTE}}}
\newcommand{\encodeindep}{{\textsf{MPW-encode}}}
\newcommand{\decodeindep}{{\textsf{MPW-decode}}}


\newcommand{\DTEsub}{{\textsf{SG-DTE}}}
\newcommand{\encodesub}{{\textsf{SG-encode}}}
\newcommand{\decodesub}{{\textsf{SG-decode}}}
\newcommand{\decodekamf}{{\textsf{KAMF-decode}}}
\newcommand{\DTEis}{{\textsf{IS-DTE}}}
\newcommand{\encodeis}{{\textsf{is-encode}}}
\newcommand{\decodeis}{{\textsf{is-decode}}}
\newcommand{\DTErej}{{\textsf{REJ-DTE}}}
\newcommand{\encoderej}{{\textsf{rej-encode}}}
\newcommand{\decoderej}{{\textsf{rej-decode}}}
\newcommand{\DTErsarej}{{\textsf{RSA-REJ-DTE}}}
\newcommand{\encodeRSAREJ}{{\textsf{rsa-rej-encode}}}
\newcommand{\decodeRSAREJ}{{\textsf{rsa-rej-decode}}}
\newcommand{\DTErsainc}{{\textsf{RSA-INC-DTE}}}
\newcommand{\encodeRSAINC}{{\textsf{rsa-inc-encode}}}
\newcommand{\decodeRSAINC}{{\textsf{rsa-inc-decode}}}
\newcommand{\DTEunf}{{\textsf{UNF-DTE}}}
\newcommand{\DTEnunf}{{\textsf{NUNF-DTE}}}


%\newcommand{\encodeis}{{\textsf{encode}_{\textrm{is}}}}
%\newcommand{\decodeis}{{\textsf{decode}_{\textrm{is}}}}
\newcommand{\rep}{\textsf{rep}}
\newcommand{\isErr}{\epsilon_{\textnormal{is}}}
\newcommand{\incErr}{\epsilon_{\textnormal{inc}}}
\def \enc {{\textsf{E}}}
\def \dec {{\textsf{D}}}
\def \SEscheme {{\textsf{SE}}}
\def \HEscheme {{\textsf{HE}}}
\def \CTR {{\textsf{CTR}}}
\def \encHE {{\textsf{HEnc}}}
\def \HIDE {{\textsf{HiaL}}}
\def \encHIDE {{\textsf{HEnc}}}
\def \decHIDE {{\textsf{HDec}}}
\def \decHE {{\textsf{HDec}}}
\def \encHEt {{\textsf{HEnc2}}}
\def \decHEt {{\textsf{HDec2}}}

\newcommand{\myind}{\hspace*{1em}}
\newcommand{\thh}{^{\textit{th}}} % th
\newcommand{\concat}{\,\|\,}
\newcommand{\dotdot}{..}
\newcommand{\emptystr}{\varepsilon}

\newcommand{\round}{\textsf{round}}

\newcommand{\alphabar}{\overline{\alpha}}
\newcommand{\numbinsbar}{\overline{b}}
\newcommand{\numballs}{a}
\newcommand{\numbins}{b}

%\def \encHE {{\sf{enc}^{HE}}}
%\def \decHE {{\sf{dec}^{HE}}}
%\def \encHEt {{\sf{enc}^{HE2}}}
%\def \decHEt {{\sf{dec}^{HE2}}}
\def \idealHE {{\mathcal{HE}}}
\def \IEnc {{\mathbf{\rho}}}
\def \IDec {{\mathbf{\rho^{-1}}}}
\def \OEnc {{\mathbf{Enc}}}
\def \ODec {{\mathbf{Dec}}}
\newcommand{\SimuProc}{\mathbf{Sim}}
\newcommand{\ROProc}{\mathbf{RO}}
\newcommand{\PrimProc}{\mathbf{Prim}}
\def \stm {g}
\def \istm {\hat{g}}
\def \kts {{f}}
\def \lex {{\sf lex}}
\def \part {part}
\def \kd {{\sf{kd}}}
\def \msgdist {{d}}
\def \keydist {{r}}
\def \ind {{\sf{index}}}
\def \kprf {z}
\def \adv {{\mathcal A}}
\def \pwds {u}
\newcommand{\mpw}{mpw}
\newcommand{\pw}{w}
\newcommand{\pwvec}{\vec{\pw}}
\newcommand{\vecx}{\vec{x}}
\def \tokens {v}
\def \calP{{\mathcal{P}}}
\def \template{{\mathcal{T}}}
\def \vaultset{{\mathcal{V}}}
\def \ext {{\sf ext}}
\def \offset {\delta}
\def \maxweight {\epsilon}
\def \advo {{\mathcal{A}}^{*}}

\newcommand{\Chall}{\textsf{Ch}}
\newcommand{\Test}{\textnormal{\textsf{Test}}}
\newcommand{\RoR}{\textsf{RoR}}
\newcommand{\MI}{\textnormal{MI}}
\providecommand{\MR}{\textnormal{MR}}
\newcommand{\MRCCA}{\textnormal{MR-CCA}}
\newcommand{\SAMP}{\textnormal{SAMP}}
\newcommand{\DTEgame}{\textnormal{SAMP}}
\newcommand{\KR}{\textnormal{KR}}
\newcommand{\advA}{{\mathcal{A}}}
\newcommand{\advR}{{\mathcal{R}}}
\newcommand{\advB}{{\mathcal{B}}} % 
\newcommand{\advC}{{\mathcal{C}}} % C
\newcommand{\advD}{{\mathcal{D}}} % D
\newcommand{\advE}{{\mathcal{E}}}
\newcommand{\advF}{{\mathcal{F}}}
\newcommand{\advG}{{\mathcal{G}}}
\newcommand{\advI}{{\mathcal{I}}}
\newcommand{\nextval}{\;;\;}
\newcommand{\TabC}{\texttt{C}}
\newcommand{\TabR}{\texttt{R}}
\newcommand{\Hash}{H}
\newcommand{\Cipher}{\pi}
\newcommand{\CipherInv}{\pi^{-1}}
\newcommand{\simu}{{\mathcal S}}
\newcommand{\prim}{P}
\newcommand{\maxguess}{\gamma}


\newcommand{\bigO}{\mathcal{O}}
\newcommand{\calG}{{\mathcal{G}}}

\def\sqed{{\hspace{5pt}\rule[-1pt]{3pt}{9pt}}}
\def\qedsym{\hspace{2pt}\rule[-1pt]{3pt}{9pt}}

\newcommand{\Colon}{{\::\;}}
\newcommand{\good}{\textsf{Good}}

\newcommand\Tvsp{\rule{0pt}{2.6ex}}
\newcommand\Bvsp{\rule[-1.2ex]{0pt}{0pt}}
\newcommand{\TabPad}{\hspace*{5pt}}
\newcommand\TabSep{@{\hspace{5pt}}|@{\hspace{5pt}}}
\newcommand\TabSepLeft{|@{\hspace{5pt}}}
\newcommand\TabSepRight{@{\hspace{5pt}}|}


\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\comma}{\textnormal{,}}

\renewcommand{\paragraph}[1]{\vspace*{6pt}\noindent\textbf{#1}\;}

\newcommand{\weirvault}{\textsf{Pastebin}\xspace}
\newcommand{\ndssvault}{\textsf{DBCBW}\xspace}




\newcommand{\reminder}[1]{ [[[ \marginpar{\mbox{$<==$}} #1 ]]] }

%
% New theorem types: (Already in CCS template)
%
\newtheorem{observation}{Observation}
%\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{fact}{Fact}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{proposition}{Proposition}
% \newtheorem{example}{Example}

%
% Definitions:
%
\def \blackslug{\hbox{\hskip 1pt \vrule width 4pt height 8pt
    depth 1.5pt \hskip 1pt}}
\def \qed{\quad\blackslug\lower 8.5pt\null\par}
% In-line QED, for ending a proof with a $$ formula
% In-line QED, for ending a proof with a $$ formula
\def \inQED{\quad\quad\blackslug}
\def \Qed{\QED}
\def \QUAD{$\Box$}
\def \Proof{\par\noindent{\bf Proof:~}}
\def \proof{\Proof}
\def \poly {\mbox{$\mathsf{poly}$}}
\def \binary {\mbox{$\mathsf{binary}$}}
\def \ones {\mbox{$\mathsf{ones}$}}
\def \rank {\mbox{$\mathsf{rank}$}}
\def \bits {\mbox{$\mathsf{bits}$}}
\def \factorial {\mbox{$\mathsf{factorial}$}}
\def \fr {\mbox{$\mathsf{fr}$}}
\def \pr {\mbox{$\mathsf{pr}$}}
\def \zon {\{0,1\}^n}
\def \zo  {\{0,1\}}
\def \zok {\{0,1\}^k}
\def \mo {s}


\def\utilcnt{\ensuremath{\mu_{\mathrm{cnt}}}}
\def\utiltime{\ensuremath{\mu_{\mathrm{time}}}}
\def\ex{\ensuremath{{\mathrm{ex}}}}
\def\rlx{\ensuremath{{\mathrm{rlx}}}}
\def\tp{\textsf{TP}}
\def\cp{\textnormal{\textsf{CP}}\xspace}
\def\edistcutoff{\edist}
\def\entcutoff{\ensuremath{m}}
\def\relentcutoff{{\sigma}}
\def\mutt{\mu_{\mathrm{tt}}}

\newcommand{\Hdot}{H(\mbox{ } \cdot \mbox{ }  , \mbox{ } \del)}


\newcounter{mynote}[section]
\newcommand{\notecolor}{blue}
\newcommand{\thenote}{\thesection.\arabic{mynote}}
\newcommand{\tnote}[1]{\refstepcounter{mynote}{\bf \textcolor{\notecolor}{$\ll$TomR~\thenote: {\sf #1}$\gg$}}}

\newcommand{\fixme}[1]{{\textcolor{red}{[FIXME: #1]}}}
\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}


\newcommand\ignore[1]{}


\newcommand\simplescheme{simple}


\newcommand{\KDF}{\mathsf{KDF}}
\newcommand{\salt}{\mathsf{sa}}
\newcommand{\PRF}{F}
\newcommand{\subgram}{\mathsf{SG}}
\newcommand{\popdomains}{\mathcal{D}}

\newcommand{\retrieve}{\textsf{Sync}}
\newcommand{\update}{\textsf{Insert}}

\newcommand{\dictW}{\textbf{D1}\xspace}
\newcommand{\dictF}{\textbf{D2}\xspace}

\newcommand{\str}{\text{str}}
\newcommand{\calS}{{\mathcal S}}

% \newcommand{\new}[1]{\textcolor{red}{\sf #1}}
\newcommand{\new}[1]{#1}


%% ------------------------- Rahul -----------------------
\newcounter{rcnote}[section]
\newcommand{\rcthenote}{\thesection.\arabic{rcnote}}
\newcommand{\rcnote}[1]{\refstepcounter{rcnote}{\bf \textcolor{magenta}{$\ll$RC~\rcthenote: {\sf #1}$\gg$}}}

\newcounter{mrnote}[section]
\newcommand{\mrthenote}{\thesection.\arabic{mrnote}}
\newcommand{\mrnote}[1]{\refstepcounter{mrnote}{\bf \textcolor{green}{$\ll$MR~\mrthenote: {\sf #1}$\gg$}}}

\newcounter{fknote}[section]
\newcommand{\fkthenote}{\thesection.\arabic{fknote}}
\newcommand{\fknote}[1]{\refstepcounter{fknote}{\bf \textcolor{blue}{$\ll$FK~\fkthenote: {\sf #1}$\gg$}}}

\newcounter{anote}[section]
\newcommand{\ajthenote}{\thesection.\arabic{anote}}
\newcommand{\anote}[1]{\refstepcounter{anote}{\bf \textcolor{cyan}{$\ll$AJ~\ajthenote: {\sf #1}$\gg$}}}



\newcommand{\mytab}{\hspace*{.4cm}}
\def\half{{1\over 2}}
\newcommand{\NT}[1]{\texttt{#1}}
\DeclareMathSymbol{\mlq}{\mathord}{operators}{``}
\DeclareMathSymbol{\mrq}{\mathord}{operators}{`'}
\newcommand{\calO}{{\mathcal O}}
\newcommand{\calA}{{\mathcal A}}
\newcommand{\kamfplus}{Kamouflage\textbf{+}\xspace}
% \newcommand{\genfrom}[1]{\;{\stackrel{\,#1}{\leftarrow}}\;}
\newcommand{\genfrom}[1]{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle#1$}}}\:}}
%\newcommand{\genfrom}[1]{\;\leftarrow{\tiny \$} #1\;}
\newcommand{\twopartdef}[4]
{
  \left\{
    \begin{array}{ll}
      #1 & \mbox{if } #2 \\[4pt]
      #3 & #4
      \end{array}
      \right.
}
\newcommand{\threepartdef}[6]
{
  \left\{
    \begin{array}{lll}
      #1 & \mbox{if } #2 \\
      #3 & \mbox{if } #4 \\
      #5 & \mbox{if } #6
      \end{array}
      \right.
}

\newcommand{\gt}[1]{\gamma_{#1,\maxdist}}
\newcommand{\gmt}[2]{\gamma_{#1,#2}}
\def\nh{\ensuremath{N}}
\def\ball{\ensuremath{B}}
\def\anh{\ensuremath{\tilde{N}_k}}
% \newcommand{\nh}[2]{{N_{#1}(#2)}}

\newcommand{\ballsizet}[1]{{\beta_{#1,\maxdist}}}
\newcommand{\ballsize}[2]{{\beta_{#1,#2}}}
\newcommand{\rh}[2]{{\bf R}_{#1, #2}}
\newcommand{\rhf}[2]{R_{f, \gamma}}
\newcommand{\realm}{{m}}
% \newcommand{\inputm}{{\tilde{m}}}
\newcommand{\lmid}{\ell_{\realm, m'}}
\newcommand{\cipherlength}{n}
\renewcommand{\SS}{\textsf{SS}}
\newcommand{\Rec}{\textsf{Rec}\xspace}
\newcommand{\rec}{\textsf{rec}\xspace}
\newcommand{\Rep}{\textsf{Rep}\xspace}
\newcommand{\Gen}{\textsf{Gen}}
\newcommand{\dis}{\textsf{dis}}

\def\chk{\textnormal{\textsf{Chk}}\xspace}
\def\reg{\textnormal{\textsf{Reg}}\xspace}
\def\exchk{\textnormal{\textsf{ExChk}}\xspace}
\def\adpchk{\textnormal{\textsf{AdpChk}}\xspace}
\def\RKROR{\textnormal{MKROR}\xspace}
\def\SRKROR{\textnormal{SKROR}\xspace}
\def\ROR{\textnormal{ROR}\xspace}
\def\ROBUST{\textnormal{ROB}\xspace}
\def\OFFDIST{\textnormal{OFFDIST}\xspace}
\def\POFFDIST{\overline{\textnormal{OFFDIST}}\xspace}
\def\OFFGUESS{\textnormal{OFFGUESS}\xspace}
\def\ONGUESS{\overline{\textnormal{ONGUESS}}\xspace}
\def\ONATTACK{\textnormal{ONATTACK}\xspace}
\def\adp{\ensuremath{\Pi\xspace}}
\def\Check{\textnormal{\textsf{Checker}}}
\def\CheckPtxt{\textnormal{\textsf{PChecker}}}
\def\trans{\textnormal{\ensuremath{T}}}
\def\transgen{\textnormal{\ensuremath{\mathcal{T}}}}
\def\pke{\ensuremath{\mathcal{E}}}
\def\pkenc{\ensuremath{\pke^{\mathrm{enc}}}}
\def\pkdec{\ensuremath{\pke^{\mathrm{dec}}}}
\def\sH{\ensuremath\mathrm{H}^s}
\def\H{\ensuremath{\mathsf{H}}\xspace}
\def\T{\ensuremath{\mathsf{T}}\xspace}
\def\W{\ensuremath{\mathsf{W}}\xspace}
\def\F{\ensuremath{\mathsf{F}}\xspace}
\def\ret{\ensuremath{\mathrm{return}}\xspace}
\def\cs{\ensuremath{t}} % Cache Size
\def\waitlen{\ensuremath{\omega}\xspace} %waitlist size
\newcommand{\M}{{\mathcal{M}}}
\newcommand{\ent}{{\bf H}}
\newcommand{\Hfuzzy}{{\mathrm{H}}^{\rm fuzz}}
\newcommand{\Hminfuzzy}{{\mathrm{H}}^{{\rm{fuzz}}}_{t,\infty}}
\newcommand{\Hpfuzzy}{{\mathrm{H}}^{{\rm{pfuzz}}}}
\newcommand{\Hinf}{{\bf H}^{{\rm \min}}_{\infty}}
\newcommand{\Hminpfuzzy}{{\bf H}^{{\rm pfuzz}}_{t,\infty}}


\def\sa{{\sf sa}}
\def\err{{\varepsilon}}%^{(e)}}}
\newcommand{\dist}{\mathcmd{p}}
\newcommand{\distest}{\hat{\mathcmd{p}}}
\newcommand{\distvec}{\mathbf{\dist}}
\newcommand{\distvecest}{\hat{\mathbf{p}}}
\newcommand{\w}{{w}}
\newcommand{\wnew}{\tilde{w}}
\newcommand{\m}{{w}}
\newcommand{\mnew}{{\tilde{m}}}
\newcommand{\mspacevec}{\mathcmd{\mathbf{W}}}
\newcommand{\mvec}{\mathcmd{\mathbf{\m}}}
\newcommand{\mvecss}[1]{\mvec_1\ldots\mvec_{#1}}
\renewcommand{\mspace}{\mathcmd{W}}
\newcommand{\mspacebot}{{\mspace}_\bot}

\newcommand{\similar}{\mathrm{sim}}
\newcommand{\similarvec}{\mathrm{\mathbf{sim}}}

\def \mvecnew{{\tilde{\mvec}}}
\newcommand{\mvecnewss}[1]{\mvecnew_1\ldots\mvecnew_{#1}}

\DeclareDocumentCommand{\edist}{o o}{
  \ensuremath{
    \IfNoValueTF{#1}{{d}}{{\sf d}(#1,#2)}
  }
}

\newcommand{\utilinc}{\mu}
\newcommand{\secloss}{\Delta}
\newcommand{\seclossg}{\Delta^\textnormal{greedy}}
\newcommand{\seclosso}{\Delta}
%\newcommand{\maxlambda}{\lambda^*}
%\newcommand{\maxfuzzlambda}{\tilde{\lambda}^*}
\newcommand{\fuzzlambda}{\lambda^\textnormal{fuzzy}}
\newcommand{\greedylambda}{\lambda^\textnormal{greedy}}
\newcommand{\greedylambdaon}{\tilde{\lambda}^\mathrm{on}}
\newcommand{\greedylambdaoff}{\tilde{\lambda}^\mathrm{off}}
\newcommand{\seclosson}{\secloss^\mathrm{on}}
\newcommand{\seclossoff}{\secloss^\mathrm{off}}
\def \edit {\ensuremath{e}}
\newcommand\error{e}
\newcommand\tab[1][1cm]{\hspace*{#1}}

\newcommand{\mathcmd}[1]{\ensuremath{#1}\xspace} % to use a command both in math mode and non-math mode
\newcommand{\minentropy}[1]{\ensuremath{\operatorname{H_\infty}\olrk{#1}}}
\newcommand{\fuzzyminentropy}[1]{\ensuremath{\operatorname{H^{fuzz}_{\maxdist, \infty}}\olrk{#1}}}
\providecommand{\condminentropy}[2]{\ensuremath{\operatorname{\tilde{H}_\infty}\olrk{#1|#2}}}
\newcommand{\s}{\mathcmd{s}}
\newcommand{\typo}{\mathcmd{\tilde{\m}}}
\newcommand{\typoj}[1]{\ensuremath{(\typo_{#1}, j_{#1})}}
\newcommand\typojprime[1]{{(\typo_{#1}, j'_{#1})}}
\renewcommand\contrib[2]{\mathsf{cont}\left[{#1}/{#2}\right]}
\def\typovec{\ensuremath{\{\typo_i\}_{i=1}}}
\def\opttypovec{\ensuremath{\{\typo^*_i\}_{i=1}}}
\def\slotguess{\textsf{SlotGuess}}
\def\typodist{\ensuremath{\tau_\pw}}
\def\cachedtypodist{\ensuremath{{\tilde{\tau}}_{\pw}}}
\def\typodistest{\ensuremath{{\hat{\tau}}_{\pw}}}
\def\incache{T_\pw}
\newcommand{\fuzzylambda}{\ensuremath{\lambda^{\mathrm{fuzzy}}}}
%\newcommand{\errorprob}[2]{\mathcmd{\tau_{#1}({#2})}}
\newcommand{\errordist}{\mathcmd{\tau}}
\newcommand{\famdist}{\mathcmd{\mathcal{W}}}
\def\guessw{\ensuremath{W}}
\newcommand{\precdist}{W}
\newcommand{\entdef}{Z}
\newcommand{\PW}{\mathcmd{\mathcal{W}}}
\newcommand{\cachedom}{\mathcmd{\mathcal{S}}}
\newcommand{\supp}{\mbox{supp}}
\newcommand{\olrk}[1]{\ifx\nursymbol#1\else\!\!\mskip4.5mu plus 0.5mu\left(\mskip0.5mu plus0.5mu #1\mskip1.5mu plus0.5mu \right)\fi}

\newcommand{\errorprob}[1]{\mathcmd{\tau_{#1}}}
\newcommand{\errorpr}[2]{\mathcmd{\errorprob{#1}{(#2)}}}
\newcommand{\Expectation}{\mathop{\mathbb E}}
\newcommand{\hash}[2]{\mathcmd{F(#1, #2)}}
\newcommand{\hashj}[3]{\mathcmd{F_{#3}(#1, #2)}}
\newcommand{\rhh}{\mathcmd{y}}
\newcommand{\x}{\mathcmd{x}}
\newcommand{\range}{\mathcmd{R}}
\newcommand{\lmm}{\mathcmd{l_\w}}
\newcommand{\rmm}{\mathcmd{r_\w}}
\newcommand{\conflict}[2]{\mathcmd{C_{#1, #2}}}
\newcommand{\Probsub}[2]{{\Pr_{#1}\left[\,{#2}\,\right]}}
\newcommand{\Condprobsub}[3]{{\Pr}_{#1}\left[\: #2\:\left|\right.\:#3\:\right]}
\newcommand{\wmid}{l_{\w, \w^\prime}}
\newcommand{\realhash}{\mathcmd{z}}
\newcommand{\collhash}{\mathcmd{z^\prime}}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor }
\newcommand{\ceiling}[1]{\left \lceil #1 \right \rceil }
\newcommand{\interval}{I}
% \newcommand{\p}[2]{p_{#1}(#2)}
\newcommand{\ssketch}{\mathcmd{\mathsf{S}}}
\newcommand{\tsketch}{\mathcmd{\msgsettingsym\mathsf{S}}}
\newcommand{\trivsketch}{\mathcmd{\tsketch_{\emptystr}}}
\newcommand{\WREC}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}REC}}}
\newcommand{\AREC}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}REC}}}
\newcommand{\WUTIL}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}UTIL}}}
\newcommand{\AUTIL}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}UTIL}}}
\newcommand{\indexset}{I}
\newcommand{\topset}{Z_1^*}
\newcommand{\cachedist}{T}
\newcommand{\pwdis}{R}
\newcommand{\onbudget}{q}
\newcommand{\blacklist}{\textsf{B}}
\newcommand{\blacklistlen}{\alpha}
\newcommand{\plaintextstate}{\bar{\state}}
\newcommand{\typocutoff}{\delta}
\newcommand{\plfuprob}{\ensuremath{\nu}}

\def\ballweight{\ensuremath{e_{\tilde{\tau}}}}
\newcommand{\Adv}{\textnormal{\textsf{Adv}}}
\newcommand{\AdvOFFLINE}[1]{\Adv^{\footnotesize\textnormal{\textrm{offdist}}}_{\footnotesize #1}}
\newcommand{\AdvOFFLINEP}[1]{\Adv^{\overline{\footnotesize\textnormal{\textrm{{offdist}}}}}_{\footnotesize #1}}
\newcommand{\AdvOFFGUESS}[1]{\Adv^{\footnotesize\textnormal{\textrm{offguess}}}_{\footnotesize #1}}
\newcommand{\AdvONGUESS}[1]{\Adv^{{\footnotesize\textnormal{\textrm{onguess}}}}_{\footnotesize #1}}
\newcommand{\AdvONATTACK}[1]{\Adv^{\footnotesize\textnormal{\textrm{onattack}}}_{\footnotesize #1}}
\newcommand{\AdvRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{mk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvSRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{sk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{ror}}}_{\footnotesize #1}}
\newcommand{\AdvROBUST}[1]{\Adv^{\footnotesize\textnormal{\textrm{rob}}}_{\footnotesize #1}}

\newcommand{\advantage}[3]{\pcnotionstyle{\Adv}^{#1}_{#2}(#3)}
\newcommand{\neighbourhood}[2]{N_{#1}({#2})}
\newcommand{\rhhdist}{Y}
\newcommand{\fullerhash}{z}
\newcommand{\errorball}[2]{{B}^{\errordist}_{#1}(#2)}
\newcommand{\f}{f}
\newcommand{\pwmaxlen}{\ell}
\newcommand{\indexi}{i}
\newcommand{\indexq}{q}
\newcommand{\indexx}{x}
\newcommand{\replace}{\textsf{replace}}
\newcommand{\vecca}{\vecc{a}}
\newcommand{\veccb}{\vecc{b}}
\newcommand{\veccv}{\vecc{v}}
\newcommand{\coins}{r}
\renewcommand{\state}{\ensuremath{\mathsf{s}}}
\newcommand{\win}{\mathsf{win}}
\newcommand{\Chk}{\textsf{Chk}}
\newcommand{\PChk}{\textsf{PChk}}
\newcommand{\indexh}{h}
\newcommand{\randomZ}{Z}
\newcommand{\Cache}{\textnormal{\textsf{Cache}}}
\newcommand{\WarmupCache}{\textnormal{\textsf{WarmupCache}}}
\newcommand{\CacheUpdate}{\textnormal{\textsf{CacheUpdt}}}
\newcommand{\CacheInit}{\textnormal{\textsf{CacheInit}}}
\newcommand{\cachestate}{\ensuremath{\mathtt{S}}\xspace}
\newcommand{\cachestatelen}{\ensuremath{\sigma}\xspace}
\newcommand{\CacheLRU}{\textnormal{\textsf{CacheLRU}}}
\newcommand{\CacheLRUUpdate}{\textnormal{\textsf{UpdateLRU}}}
\newcommand{\CacheLRUInit}{\textnormal{\textsf{InitLRU}}}


\newcommand{\zxcvbn}{\textnormal{\textsf{zxcvbn}}\xspace}
\newcommand{\bad}{\textnormal{\textsf{bad}}}
\newcommand{\wait}{z}
\newcommand{\PKE}{\textnormal{\textsf{PKE}}}
\newcommand{\pkegen}{\mathcal{K}}
\newcommand{\pkeenc}{\mathcal{E}}
\newcommand{\pkedec}{\mathcal{D}}
\newcommand{\pkectxtspace}{\mathcal{C}_{\pkeenc}}
\newcommand{\pk}{{pk}}
\newcommand{\sk}{{sk}}
\newcommand{\PBE}{\textnormal{\textsf{PBE}}}
\newcommand{\utility}{\textsf{Utility}}

\newcommand{\skegen}{\ensuremath{\mathsf{K}}}
\newcommand{\skeenc}{\ensuremath{\mathsf{E}}}
\newcommand{\skedec}{\ensuremath{\mathsf{D}}}
\newcommand{\skectxtspace}{\ensuremath{\mathcal{C}_{\skeenc}}}
\newcommand{\ske}{\textnormal{\textsf{SKE}}}
\newcommand{\SE}{\textnormal{\textsf{SE}}}
\newcommand{\sekg}{\mathcal{K}}
\newcommand{\seenc}{\mathcal{E}}
\newcommand{\sedec}{\mathcal{D}}
\newcommand{\saltlen}{{\ell_{\mathrm{salt}}}}

\newcommand{\skk}{\textnormal{\textsf{k}}}
\newcommand{\cipherske}{{c}}
\newcommand{\cipherpke}{{c}}
\newcommand{\SH}{\textnormal{\textsf{SH}}}
\newcommand{\FH}{\textnormal{\textsf{H}}}
\newcommand{\counter}{\textnormal{\textsf{Count}}}
\newcommand{\indexp}{p}
\newcommand{\ciphertextspace}{\mathcal{C}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\indexr}{r}
\newcommand{\vecc}[1]{\mathbf{#1}}
\newcommand{\sawait}{\overline{\sa}}
\newcommand{\skkwait}{\overline{\skk}}
\newcommand{\hwait}{\overline{\indexh}}
\newcommand{\randomY}{Y}
\newcommand{\indexm}{m}
\newcommand{\hashtable}[1]{H[#1]}
\newcommand{\SHlen}{k_1}
\newcommand{\FHlen}{k_2}
\newcommand{\valid}{\textnormal{\textsf{valid}}}
\newcommand{\skepsilon}{\epsilon_{ske}}
\newcommand{\pkepsilon}{\epsilon_{pke}}
\newcommand{\hybindex}{j}

\newcommand{\DL}{\textnormal{DL}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\indicator}{\mathbb{I}}
\newcommand{\cipherspace}{\mathcal{C}}
\newcommand{\pkemsgspace}{\mathcal{M}_\pkeenc}

\newcommand{\pkecipher}{c}
\newcommand{\skecipher}{{c}}
\newcommand{\pkemsg}{m}
\newcommand{\skemsg}{{m}}
\newcommand{\skemsgspace}{ \msgspace_{\skeenc}}
\newcommand{\upperb}{\alpha}

\newcommand{\ffbox}[1]{
   \setlength{\fboxsep}{-1\fboxrule}
   \fbox{\hspace{1.2pt}\strut#1\hspace{1.2pt}}}


\newcommand{\statespace}{S}
\newcommand{\targuess}{\textsf{TarGuess}}
\newcommand{\untarguess}{\textsf{UnTarGuess}}

\newcommand{\accept}{\texttt{accept}}
\newcommand{\reject}{\texttt{reject}}
\newcommand{\threshold}{\ensuremath{\tau}}
\newcommand{\clfthreshold}{\ensuremath{\theta}}
\newcommand{\far}{\ensuremath{\alpha}}
\newcommand{\frr}{\ensuremath{\beta}}
\newcommand{\fpr}{\ensuremath{\nu}}
\newcommand{\fnr}{\ensuremath{\gamma}}
\newcommand{\FPR}{\textrm{FPR}}
\newcommand{\FNR}{\textrm{FNR}}


\newcommand{\matchalgo}{\mathcal{L}}
\newcommand{\matchalgovec}{\mathcal{\mathbf{L}}_\sslen}
\def \score {\theta}
\newcommand{\indexjvec}{\ensuremath{\mathcmd{\mathbf{j}}\xspace}}
\def\k{k}
\newcommand{\add}{\funcfont{Add}}
\newcommand{\accuracy}{\funcfont{Accuracy}}
\def\acc{\delta}
\def \MS {\funcfont{MS}}
\def \MRec {\funcfont{MRec}}
\newcommand \MSt{\MS^{\matchalgo}_\sslen}
\newcommand \MRect{\MRec^{\matchalgo}_\sslen}
\def \nmatches {\ensuremath{l}}
\def \D{D}
\def \Dmod{\tilde{D}}
\def \mlen{n}
\def \sslen{t}
\def \secret{s}
\def \secretvec{\mathbf{s}}
\newcommand{\sketch}{{\funcfont{sketch}}}
\newcommand{\sketchval}{v}
\def \recover{\funcfont{recover}}
\def \verify{\funcfont{verify}}
\def \q{q}
\def\fp{\alpha}
\def\fn{\beta}
\def\tp{\gamma}
\newcommand{\one}{\ensuremath{\mathbbm{1}}}
\newcommand{\seclen}{\ell}
\newcommand{\Overify}{{\mathcal{O}_\funcfont{vrfy}}}
\newcommand{\Omatch}{\mathcal{O}_\funcfont{match}}
\newcommand{\ith}[2]{#1_{#2}}
\newcommand{\jth}[2]{#1^{#2}}
\newcommand{\mspacei}{\ith{\mspace}{i}}
\newcommand{\errori}{\ith{\error}{i}}
\newcommand{\matchalgoi}{\ith{\matchalgo}{i}}
\newcommand{\mvecbar}{\overline{\mvec}}
\newcommand{\mvectilde}{\tilde{\mvec}}
\newcommand{\angbrac}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\clf}{\mathcal{C}}
\newcommand{\clft}{\clf_\sslen}
\newcommand{\clfest}{\mathcal{\hat{\clf}}}
\newcommand{\clfq}[1]{{\clf^q_{#1}}}
\newcommand{\nclf}{r}
\newcommand{\oclf}{\omega}
\newcommand{\biosketch}{\funcfont{TenSketch}\xspace}
\newcommand{\tensketch}{\funcfont{TenSketch}\xspace}

\newcommand{\hvec}{\mathbf{h}}
\newcommand{\insertr}{\mathsf{insert{\scriptstyle\$}}}
\newcommand{\dbmsg}{\ensuremath{\mathcal{F}}}
\newcommand{\dbmsgs}{\ensuremath{\{\dbmsg_i\}}}
\newcommand{\dbid}{\mathcal{I}}
\newcommand{\db}{\ensuremath{D}}
% \newcommand{\dbs}{\ensuremath(\dbid,\{\dbmsg_i\})}
\newcommand{\dbs}{\ensuremath(\dbid,\dbmsg)}
\newcommand{\dbsprime}{\ensuremath(\dbid',\dbmsg')}
\newcommand{\dbsize}{N}
\def \dblen{N}
\def\mhat{\hat{\mvec}}
\def\findmatches{\funcfont{\footnotesize FindMatches$^{\matchalgo}$}}
\newcommand{\setss}[1]{\SS^\Delta_{#1}}
\newcommand{\setrec}[1]{\Rec^\Delta_{#1}}
\newcommand{\setsst}{\setss{\sslen}}
\newcommand{\setrect}{\setrec{\sslen}}
\newcommand{\costs}{{c_s}}
\newcommand{\costc}{{c_c}}
\NewDocumentCommand{\indseq}{ O{1} O{r} }{{#1}\ldots {#2}}
\newcommand{\seq}[2]{{{#1}_1,\ldots,{#1}_{#2}}}
\newcommand{\relu}{\funcfont{ReLu}}
\newcommand{\fcrelu}[1]{\funcfont{FC}_{\relu}^{#1}}
\newcommand{\gencliq}{\funcfont{GenTupIncr}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Recent developments in smart contract security have advanced towards a wide array of learning-based dynamic analyses, with impressive results achieved by hybrid fuzzing \cite{fuzzingsurvey, concolicexe, learnedfuzzing}. In particular. While concolic-execution-assisted hybrid fuzzing is highly effective at exploring challenging program paths, %\kexin{I think concolic execution cannot explore *all* paths maybe tone down a bit?},
it often requires substantial computational resources, such as intensive usage of CPU and memory to track and solve path constraints. Given that no single technique is perfect and to better support concolic execution assisted fuzzing, this begets the \emph{scalability question}: what if we can automatically forecast the right technique to use before heavily investing scarce computational resources?  
%\kexin{I think fuzzing and concolic execution are not used alone in history, so do we need to formulate the problem as deciding between fuzzing and concolic? IIRC, many fuzzers when we worked on Neuzz were based on concolic execution and taint analysis. is it rare in smart contracts? maybe argue a little bit about why people have not tried smart contracts here.}

In addition to resource constraints, new studies show that bugs are often deeply embedded in execution paths \cite{arbiter}, and more importantly, detecting such ``deep bugs'' requires writing fuzz targets that can correctly capture the underlying transactional logic. Prior to foundation models, it behooves developers to spend hours, if not days, on writing fuzz targets. 
Recently, foundation models have been used to automate fuzz target generation \cite{llm4fuzz, llamafuzz, fuzz4all} by leveraging their code understanding and generation capabilities.
%\jianan{It seems that the three papers cited here use LLMs for classical fuzzing rather than hybrid fuzzing. I scanned through them and didn't find how their fuzzing integrated concolic execution (maybe I missed them). How about the following? "Recently, foundation models have been used to automate fuzz target generation by leveraging their code understanding and generation capabilities."}
However, hallucination results in syntactically incorrect fuzz targets that still require manual fixes. 
This limitation begets the \emph{correctness question}:
%\kexin{why do we call low-quality fuzz target ``unsound''? it sounds to me soundness are more on how you consider all execution paths, basically dynamic analysis is not sound as it focuses on single path at a time}: 
how do we suppress syntactical errors while generating effective (defined as syntactically correct and ``deep bug'' reachable) fuzz targets?
\junfeng{if by hallucination all we mean are the compilation errors, then perhaps be more direct to call them syntactical and semantic errors, and refer to hallucination less in the rest of the paper}

Our research seeks to address the scalability and correctness questions in real-world smart contract applications.
While current advances offer promising directions, limited scalability and hallucination are key performance bottlenecks hindering further progress. Scalable techniques like randomized fuzzing often suffer from low code coverage and consequently a low bug detection rate, as fuzzers generating random inputs tend to get trapped in constrained paths.\junfeng{not sure 'constrained paths' are accurate; randomized fuzzing has problems exploring constrained paths} High code coverage analyses, such concolic execution, often come at the price of limited scalability. Their exhaustive path searches are either narrowly focused on a limited code subset or require exponentially increasing amounts of memory space\junfeng{is it just memory space or more generally cpu time as well?} \cite{pathexplosion}.

To mitigate the trade-off between scalability and coverage, the software testing community has devoted much energy to writing effective fuzz targets \cite{fudge, utopia,where2fuzz}.  Foundation-model-based tools have shown significant promise in automating fuzz target generation at scale at Google OSS-Fuzz \cite{ossfuzz}.  Despite the initial efforts, the coverage improvement and bug detection results are curtailed by hallucinated foundation models' output. Our internal analysis shows that hallucination prevents 21 out of 27 tested smart contract benchmarks \cite{efcf, echidna} from meaningful coverage improvement, because incorrect fuzz targets invariably require human inspection and several rounds of manual fixes. 


To achieve high scalability, our \textbf{first insight} is to let a technique do what it's best at: a technique is most effective when it incorporates domain-specific knowledge to automatically detect bugs that fall within its strength. The challenge is to know in advance which code segments of a smart contract is best suited for a given technique\junfeng{what are the techniques to pick from? randomized fuzzing vs concolic execution, right? If so we should be explicit}. To that end, we introduce a forecast model that interacts with dynamic analysis and a fuzz target generator model. Forecasting first increases scalability by reducing futile techniques' runtime.

\sally{LLMs are useful, because it has enlarged search space ...}

To suppress hallucination of the fuzz target generator model, our \textbf{second insight} is that foundation models are receptive to feedback from compilers and other techniques. Feedback from compilers, such as error messages, and from other techniques, such as coverage data, enhance foundation models' code generating ability by giving foundation models a chance to automatically fix the errors of generated fuzz targets with concrete error points and contexts. What diff\junfeng{there are code editting models that can incoprorate feedback. we may want to cite and differentiate} 

%To unify the strengths of dynamic analysis and foundation models, our \textbf{third insight} is that a system should serve its users by self-deciding the right technique and self-correcting hallucination-induced errors. We observe that when the parts of a system, such as fuzzing, concolic execution, and foundation models, learn to interact with each other, the interactions produce greater synergies (defined as code coverage and bug detection results) than the sum of its parts.\junfeng{not clear to me the value of this insight} 

We demonstrate that it's feasible to achieve high scalability with suppressed hallucination by introducing \sys. We evaluated \sys on real-world smart contract benchmarks. Evaluation shows that compared to similar tools and baselines, \sys generates hallucination-free fuzz targets and improves coverage by up to 14.3\% on those benchmarks. Interestingly, \sys has discovered a critical vulnerability that has escaped eleven existing tools for more than a year. Anonymized artifacts and reproducing code are available \footnote{https://anonymous.4open.science/r/SCTest-5F4C/algo/executor/corpus}.
%\junfeng{has the bug been confirmed? if not, please try to follow up and get the bug confirmed.}
% \begin{scriptsize}
 \mycode
\begin{lstlisting}[float,floatplacement=H,basicstyle=\fontsize{8}{9}\selectfont, caption={{P1. Common bottleneck for fuzzing: CVE-2023-34234 (simplified for readability).}}, label={fuzzingexample},numbers=left, xleftmargin=2em]
function castVote(uint id, address voter, string calldata reason, bytes memory params. bytes memory sig) external returns (bytes) {
  //challenge: magic number constraints
  if (abi.encode(voter, id)==keccak256(abi.encode(bytes(reason), params, sig))) {
      _castVoteInternal(...); //buggy call
  }
  revert()
}
...
\end{lstlisting}
% \end{scriptsize}

\vspace{.1cm}\noindent\textbf{Contributions.} We make the following contributions:
\begin{itemize}[leftmargin=*]
\item To the best of our knowledge, \sys is the first interactive, self-deciding system that achieves high scalability while generating hallucination-free fuzz targets to detect ``deep bugs'' in real-world smart contracts.
\item \sys taps into foundation models'  forecasting power via augmented code understanding ability, generating test cases that consistently improve \efcf's coverage, an AFL++ adapted fuzzer for Solidity, on sampled 82 projects.

\item We present a trio of comprehensive benchmarks useful for fine-tuning, coverage, and bug detection analyses. The benchmark is comprised of the top five types of commonly exploited zero-day vulnerabilities from 2022-2024. 
%\jianan{Do you create three separate benchmarks or one benchmark with different components? Right now "we present a trio" indicates separate benchmarks, while "the benchmark is comprised of" (rather than "the benchmarks are") suggests one unified benchmark.}

\end{itemize}


==> overview.tex <==
\section{Overview}
\label{sec:overview}


Fig.~\ref{Fig:overview} illustrates our efforts to build such an interactive system and the workflow of \sys. During fine-tuning, the fuzz scanner generates coverage reports from training contracts (\textcircled{\footnotesize{1}}). \sys automatically processes these reports to fine-tune the forecast model. Once the forecast model is fully fine-tuned (\textcircled{\footnotesize{2}}), \sys takes  \textbf{a previously unseen contract as input}. After the fuzz scanner generates a coverage report, \sys calls the forecast model (\textcircled{\footnotesize{3}}). Then the forecast model decides whether to invoke concolic execution (forecast output as 1) or the generator model (forecast output as 0) (\textcircled{\footnotesize{4}}). If the generator model is invoked, \sys applies hallucination suppression algorithm (\textcircled{\footnotesize{5}}) and feeds corrected fuzz targets back into the fuzz scanner (\textcircled{\footnotesize{6}}). \sys repeats this process until coverage plateaus or the fuzz scanner time outs. If concolic execution is invoked, \sys uses concolic execution to overcome coverage plateaus. Eventually, \sys generates \textbf{test cases (possible exploits) as output} (\textcircled{\footnotesize{7}}). 
%Specifically, \sys's interactive modules are the following: 

\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{Fig/workflow.pdf}
\caption{\sys's workflow}
\label{Fig:overview}
\end{figure}

%\vspace{0.1cm}\noindent\textbf{Forecast Model.} The fine-tuned model takes coverage report and smart contract source code as input and predicts the next module \ie concolic execution or generator model, as output. If the forecast model predicts 0 (meaning that the model predicts concolic execution as a befitting module to overcome the coverage plateaus), \sys proceeds to the concolic execution module as a next step. If the forecast model predicts 1 (meaning that the model predicts foundation model as a befitting module to overcome the coverage plateaus), \sys proceeds to prompt the generator model as the next step to generate test targets (details in \S\ref{subsec: fine-tuned Binary Classification Model}).
%\sys employs different default foundation models for binary classification and test case generation for optimal performance. The technical rationale and performance-based evidence for such design choice are detailed in \ref{subsec: Finetuned Binary Classification Model}. 

%\vspace{0.1cm}\noindent\textbf{Optimized Concolic Execution.} To escape coverage plateaus, \sys employs coverage-guided concolic execution to generate test cases with real-time coverage monitoring. This module takes a smart contract, initial corpus, and coverage report as input and returns new test cases and updated coverage as output. Although concolic (or symbolic) execution has been widely used for test case generation in other domains such as C and Java \cite{Klee, ucklee, dart, multise}, Ethereum smart contracts and solidity require technical optimizations to maximize coverage and to overcome the bottlenecks in \S\ref{subsec:coomon_bottlenecks}.

%\vspace{0.1cm}\noindent\textbf{Generator Model.} The fuzz target generator model takes smart contract source code and coverage report as input and generates fuzz targets as output. When \sys prompts the model, the goals are: i) to generate fuzz targets that can maximize coverage for the uncovered functions; ii) to generate fuzz targets with specific function invocation orders that can discover hidden bugs. After extracting specific function invocation orders and functions not covered by initial fuzzing, fuzz target generation and hallucination suppression are in \S\ref{subsec: Test Case Generation Model} and \S\ref{subsec: hallucination suppression algorithm}.
%\kexin{step 6: justify LLM or symbolic execution makes sense; separate function invocation order and input value generation; if we use a fixed function and not efficient; else: if we need function invocation orders and efficienty; reverse explaining: after training, we discover that LLMs are good at identifying invocation order and more efficient covering constraints test case. When we have multiple function invocation order, predicting 1.}
